Collimating cylindrical Surface Leaky Waves for Highly Improved Radiation Characteristics of Holograms

High resolution microwave leaky wave holograms excited by center-fed cylindrical surface wave launcher show a null at object wave direction which is an undesired effect for electromagnetic beamforming. Also, planar leaky wave metasurfaces generating a tilted beam extremely suffer from the destructive effect of non-forward surface leaky waves at frequencies other than the design frequency and they are almost operable at a single frequency. Here we propose a 2-D modified hologram configuration using parabolic surface reflector to collimate the non-forward leaky modes into the forward leaky modes. The modified hologram presents null-free radiation pattern and highly improved operating frequency bandwidth. The consequent frequency bandwidth provides the scannabality property by frequency variation. The forward mode-dominant surface wave excitation of hologram lets the metasurface to generate the object beam more precisely; therefore, high directivity all over the operating bandwidth is obtained. The parabolic reflector lets the radiative surface of the metasurface to get shrunken in less than half of the conventional holograms. The concept is verified by fabrication and experimentally tested confirming the beam maintenance over a reasonable frequency range and scannability property.

==> TEMP.tex <==
\subsubsection{Wave Leakage Analysis}
The surface wave traveling on a dielectric shows properties which can be utilized for wave leakage engineering\cite{barone,barone2,cassedy,tamir}
The knowledge of dispersion diagram of a modulated, periodic, surface wave guiding structure provides an insight into the spatial harmonics allowed to radiate and angle scanning by frequency variation. In the dispersion diagram the region $k_0a/\beta a>1$ is fast wave region(stands for greater phase velocity than the speed of light) which indicates the region wave radiation is allowed and the wave leakage necessities are satisfied for all $n^{th}$ spatial harmonics placed at this region.

A lossless dielectric-filled waveguiding line of relative permittivity $\sqrt{\epsilon_r}>1$  represents a slightly deviated dispersion line for the $n=0$ mode compared to the $k_0a/\beta a=1$ line toward the bounded region. 
The dispersion curve for the modes can be obtained by shifting the $n=0$ mode curve to $\beta d=2n\pi$ for each mode. By loading the waveguide with the surface impedance surface on top, the dispersion curve slightly gets departed for the $k_0a/\beta a=1/\sqrt{\epsilon_r}$ (see FIG. 6).


\begin{figure}[H]
\includegraphics[width=1\linewidth]{dispersion_diagram.png}
\caption{The leaky}
\label{fig:fig02}
\end{figure}


In a sinuously modulated surface impedance about an average value supporting $TM$ surface wave, the periodic space-varying behavior of the surface impedance boundaries provides spatial harmonics expansion for the wave leaving the modulated surface at an infinitesimally distance above the surface. The Bloch wave number $\kappa$ (fundamental tangential wave number) may be obtained through a continued fraction in $(9)$\cite{oliner}. \color{red}NOTICE WHY n=-1?\color{black}
\begin{equation}
\label{eq:eq10}
\begin{split}
1-\frac{j}{X_0} \sqrt{1 - (\frac{\kappa}{k_0})^2}=\\
&\frac{\qquad \quad \quad\frac{M^2}{4}\qquad \quad \qquad |}{1-\frac{j}{X_0}\sqrt{1-[\frac{\kappa}{k_0}+\frac{2\pi(-1)}{k_0a}]^2}}
 \\
&- \frac{\qquad \quad \quad\frac{M^2}{4}\qquad \quad \qquad |}{1-\frac{j}{X_0}\sqrt{1-[\frac{\kappa}{k_0}+\frac{2\pi(-2)}{k_0a}]^2}}...
\\
&+ \frac{\qquad \quad \quad\frac{M^2}{4}\qquad \quad \qquad |}{1-\frac{j}{X_0}\sqrt{1-[\frac{\kappa}{k_0}+\frac{2\pi(+1)}{k_0a}]^2}}
\\
&- \frac{\qquad \quad \quad\frac{M^2}{4}\qquad \quad \qquad |}{1-\frac{j}{X_0}\sqrt{1-[\frac{\kappa}{k_0}+\frac{2\pi(+2)}{k_0a}]^2}}...
\end{split}
\end{equation}
Where $X_0$ indicates normalized average surface impedance with respect to the free-space wave impedance. $\kappa$ includes both real imaginary values $(\beta-j\alpha)$. Assuming the surface impedance unmodulated $(M=0)$, the equation gives the attenuation-free wave number $\kappa=k_0\sqrt{1+X_0^2}$, implying fully coupled to surface wave with no leakage(radiation). For small enough values of $M$ the equation $(9)$ can be rewritten as:
\begin{equation}
\label{eq:eq10}
\begin{split}
\beta-j\alpha=k_0\sqrt{1+X_0^2}-\frac{M^2}{4}\frac{k_0X_0^2}{\sqrt{1+X_0^2}}\qquad \quad \quad\quad\quad
\\
\times[\frac{1}{1-\frac{j}{X_0}\sqrt{1-(\sqrt{1+X_0^2}-\frac{2\pi}{k_0a})^2}}
\\
+\frac{1}{1-\frac{j}{X_0}\sqrt{1-(\sqrt{1+X_0^2}+\frac{2\pi}{k_0a})^2}}]
\end{split}
\end{equation}

The direction which the surface impedance allows the surface wave to leak is predominantly controlled by $X_0$ and $alpha$. Considering the equation $(11)$, with a proper choice of $X_0$ or $alpha$ the other one will be defined for a desired object wave direction.
\begin{equation}
\label{eq:eq11}
\sin{\theta_{n=-1}}=\sqrt{1+X_0^2}-\frac{2\pi}{k_0a}
\end{equation}
The modulation factor $M$ determines the depth of sinuously space-dependent variations about the average surface impedance and it controls the attenuation constant $\alpha$. By defining M on low values, the surface wave obtains enough travel length on the surface and gradual wave leaking with proper accuracy. In contrast, choosing high values for M and consequent larger sinuously variations on the modulated surface make the surface wave leave the surface in a short amount of length that the surface wave travels on. Therefore, the leaking procedure does not acquire enough space and time to form the object wave with desired accuracy. High side-lobe levels are observed in this case. We chose $M=0.35$ for our application. Since the parabolic reflector-enabled leaky wave metasurface collimates the surface wave, the surface leaky wave can be treated as a bundle of unidirectional forward surface leaky waves. The radiation directivity fo such a structure is\cite{collin}: 
\begin{equation}
\label{eq:eq12}
D\propto \frac{\beta_\parallel}{\alpha_\bot}=\frac{\sqrt{\omega^2\mu_0\epsilon_0-(\kappa-\frac{2\pi}{d})^2}}{\alpha_\bot} 
\end{equation}
As the modulation factor $M$ increases, the surface wave tends to radiate sooner while traveling on the metasurface and the attenuation constant $\alpha$ increases, which causes lower directivity value and object wave accuracy. Therefore, higher side-lobe levels are expected while the antenna scans the elevation angle.
To illustrate the concept some radiation characteristics of the conventional and proposed parabolic reflector-enabled holographic metasurface radiator both fed by cylindrical surface wave launchers are compared. The object wave direction and design frequency are assumed to be $\theta_0=70^{\circ}$ and $f_0=18GHz$  for both holograms. This selection of $\theta_0$ provides scanning property by frequency decrease.
To compare the effect of non-forward surface leaky waves on hologram operating bandwidth, the distributed 2-D radiation patterns at $f=17GHz$ are posed in Fig.\ref{pattern_comparision_17GHz} . Both holograms use hexagonal unit-cells to realize the surface impedance.
 \begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{pattern_comparision_17GHz.png}
\caption{Comparison of simulated\cite{CST} 2-D patterns of conventional$(a)$ and parabolic reflector-enabled$(b)$ holographic radiators at $f_0 -\delta f(17GHz)$.}
\label{pattern_comparision_17GHz}
\end{figure}
As it is clear in Fig.\ref{pattern_comparision_17GHz}, the non-forward surface leaky waves significant destructive effect on the object wave make the radiation pattern unacceptable for the conventional hologram. In contrast, the hologram using parabolic reflector by redirecting the non-forward surface leaky waves into forward ones achieves a main-lobe magnitude of $22.9dB$ and $9.5dB$ for side-lobe level at $f=17GHz$. Fig.\ref{directivity_frequency}  illustrates  how the proposed hologram remains highly directive over $13-18GHz$.
\textbf{\begin{figure}[H]
\centering
\includegraphics[width=0.9\linewidth]{Gain.png}
\caption{Full-wave simulation of the conventional and proposed holograms with respect to frequency.}
\label{directivity_frequency}
\end{figure}}

By lowering the operating frequency, the hologram tends to scan $\theta$ angle and $\theta_{scan}=60.0^{\circ}$ is obtained for $f=17GHz$
